DaGAN++: Depth-Aware Generative Adversarial Network for Talking Head Video Generation

Predominant techniques on talking head generation largely depend on 2D information, including facial appearances and motions from input face images. Nevertheless, dense 3D facial geometry, such as pixel-wise depth, plays a critical role in constructing accurate 3D facial structures and suppressing complex background noises for generation. However, dense 3D annotations for facial videos is prohibitively costly to obtain. In this work, firstly, we present a novel self-supervised method for learning dense 3D facial geometry (ie, depth) from face videos, without requiring camera parameters and 3D geometry annotations in training. We further propose a strategy to learn pixel-level uncertainties to perceive more reliable rigid-motion pixels for geometry learning. Secondly, we design an effective geometry-guided facial keypoint estimation module, providing accurate keypoints for generating motion fields. Lastly, we develop a 3D-aware cross-modal (ie, appearance and depth) attention mechanism, which can be applied to each generation layer, to capture facial geometries in a coarse-to-fine manner. Extensive experiments are conducted on three challenging benchmarks (ie, VoxCeleb1, VoxCeleb2, and HDTF). The results demonstrate that our proposed framework can generate highly realistic-looking reenacted talking videos, with new state-of-the-art performances established on these benchmarks. The codes and trained models are publicly available on the GitHub project page at https://github.com/harlanhong/CVPR2022-DaGAN

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> context/coverletter.tex <==

\noindent Dear Editor and Reviewers,

\noindent We are submitting our manuscript entitled ``DaGAN++: Depth-Aware Generative Adversarial Network for Talking Head Video Generation‘‘ for consideration to IEEE Transactions on Pattern Analysis and Machine Intelligence. This paper extends our work which was published at previously. With respect to the conference version, the main difference includes:

\begin{itemize}
    \item To capture the accurate face expression, we propose an improved face depth network to estimate the accurate face depth map in an unsupervised fashion and utilize a geometry-enhanced multi-layer generation process to incorporate the geometry information into the generation process. In all experiments, we demonstrate the boosting performance from the proposed method (see Table~\ref{tab:same-vox1},~\ref{tab:same-hdtf},~\ref{tab:same-vox2},~\ref{tab:abla})
    \item We conduct extensive new experiments on another two popular datasets on these tasks (\ie, HDTF (Figure~\ref{fig:cross-hdtf} and Table~\ref{tab:same-hdtf}) and Voxcelebv2 (Table~\ref{tab:same-vox2})). We validate the effectiveness of the proposed model on all datasets, showing superior performance compared with the state-of-the-art methods. We also compared the geometry-enhanced feature with the geometry-free feature to verify the effectiveness of the introduction of geometry information.
    \item We enrich the related works, provide more technical details of the proposed approach and significantly expand the experimental results and analysis.
\end{itemize}

\noindent The research highlights are listed as follows.
\begin{itemize}
   \item To the best of our knowledge, our work is the first to introduce a self-supervised learning approach for recovering explicit dense 3D geometry (\ie, depth maps) from face videos for talking head video generation, leveraging the learned depth to enhance performance.

    \item We propose an innovative depth-aware generative adversarial network (DaGAN) for talking head generation, effectively integrating depth information into the generation network through two meticulously designed mechanisms: depth-guided facial keypoint estimation and cross-modal (\ie, depth and image) attention learning. We extend DaGAN by developing an advanced facial depth network capable of producing more accurate depth maps, which bolsters talking head generation, and by designing a geometry-enhanced multi-layer module that controls facial structure message passing among features of varying scales.

    \item Lastly, we conduct extensive experiments on three distinct, challenging datasets, demonstrating that our proposed model significantly surpasses previous methods by incorporating more precise geometry information and exhibits highly competitive performance across all datasets compared to state-of-the-art techniques.
\end{itemize}

\par\noindent Sincerely,

\par\noindent Fa-Ting Hong, Dan Xu
\par\noindent Department of Computer Science and Engineering, HKUST
\par\noindent Email:fhongac@cse.ust.hk, danxu@cse.ust.hk

==> coverlt.tex <==
%
% SHUletter.cls -- a document class for writing letters with OSU letterhead 
% This class based on "Fudan Recommendation Letter Template" in 2021, Nesime Tatbul (tatbul@cs.brown.edu)
%
%	
% The SHU version modificated by Zhendong Li
% (zhendong.li2001@outlook.com), 23 Nov 2022
% Notes:
%
% 1. This class can be used for creating letters with SHU logo at the
%    header and  department address at the footer 
% 2. It is based on the standard Latex document class, letter.cls.
% 3. Required packages are epsfig and ifthen.
% 4. If SHU logo is to be included in the head, then the file
%    shu.eps must be provided. Otherwise, the logo is omitted.
%

\NeedsTeXFormat{LaTeX2e}
\ProvidesClass{THUletter}
\RequirePackage{graphicx}
\RequirePackage{epstopdf}
\RequirePackage{epsfig}
\RequirePackage{ifthen}
\RequirePackage{xcolor}
\definecolor{slcolor}{HTML}{B908C5}
%\RequirePackage{fontspec}
\DeclareGraphicsExtensions {.png, .pdf}

\DeclareOption*{\PassOptionsToClass{\CurrentOption}{letter}}
\ProcessOptions
\LoadClass[letterpaper]{letter} % we always use letter paper

\newcommand{\subjectname}{Subject}
\newcommand{\@subject}{}
\newcommand{\subject}[1]{\renewcommand{\@subject}{\subjectname: #1}}

\newboolean{logofound}
\IfFileExists{THUlogo.eps}
    {\setboolean{logofound}{true}}
    {\setboolean{logofound}{false}}

\setlength{\textwidth}{6.875in}
\setlength{\textheight}{7.0in}
\setlength{\topskip}{0.0in}
\setlength{\footskip}{1.0in}
\setlength{\oddsidemargin}{-0.25in}
\setlength{\evensidemargin}{-0.25in}
\setlength{\topmargin}{-0.875in}

\DeclareFixedFont{\xcmrbn}{OT1}{cmr}{b}{n}{10}
\DeclareFixedFont{\xcmrmn}{OT1}{cmr}{m}{n}{10}
\DeclareFixedFont{\ixcmrmn}{OT1}{cmr}{m}{n}{9}

\newsavebox{\departmenthead}
\newsavebox{\departmentfoot}
\newsavebox{\emptyfoot}

\sbox{\departmenthead}{
    \begin{tabular*}{\textwidth}
                    {@{}l@{\extracolsep{0.0in}}|@{\extracolsep{0.125in}}l@{}}           

% HELP FOR SETTING UP PARBOXES
% \parbox[position][height][inner-pos]{width}{text}
% The \parbox has two mandatory arguments:
%     width - specifies the width of the parbox, and
%     text - the text that goes inside the parbox. 
% LaTeX will position a parbox so its center lines up with the center of the text line. The optional position argument allows you to line up either the top or bottom line in the parbox (default is top).
% If the height argument is not given, the box will have the natural height of the text.
% The inner-pos argument controls the placement of the text inside the box. If it is not specified, position is used.
%     t -- text is placed at the top of the box.
%     c -- text is centred in the box.
%     b -- text is placed at the bottom of the box.
%LOGO
%
%     \parbox{4.00in}
%     {\raggedright
%         \ifthenelse{\boolean{logofound}}
%            {\epsfig{file=THUlogo.eps, width=3.9in, height=1.4in}}
%            {\parbox[c][2.0in][c]{6.0in}{\hfill} 
%             \ClassWarning{THUletter}{thu.eps COULD NOT BE FOUND!}}
%     } &
% %DEPARTMENT OR SCHOOL
% %  This just sets the size of the box to the right of the logo, and the size of the vertical line.  The vertical line is set by the size of the first numerical argument of the \parbox command.
% %
% % In the future, the "From" address might be better set using "tikz".
%     \parbox[c][1.8in][c]{2.225in}{{~}\\
% }\\
%     \end{tabular*}
% }

\savebox{\emptyfoot}[\textwidth][c]{\ixcmrmn
    \hspace*{\textwidth}
}

% header and footer should be placed only on the first page
\renewcommand{\ps@firstpage}{
    \setlength{\headheight}{1.375in}
    \setlength{\headsep}{1.0in}
    \renewcommand{\@oddhead}{\usebox{\departmenthead}}
    \renewcommand{\@oddfoot}{\usebox{\departmentfoot}}
    \renewcommand{\@evenhead}{}
    \renewcommand{\@evenfoot}{}
}

\renewcommand{\ps@empty}{
    \setlength{\headheight}{1.375in}
    \setlength{\headsep}{0.5in}
    \renewcommand{\@oddhead}{}
    \renewcommand{\@oddfoot}{\usebox{\emptyfoot}}
    \renewcommand{\@evenhead}{}
    \renewcommand{\@evenfoot}{\usebox{\emptyfoot}}
}

\providecommand{\@evenhead}{}
\providecommand{\@oddhead}{}
\providecommand{\@evenfoot}{}
\providecommand{\@oddfoot}{}

\pagestyle{empty}

% we add the subject command to the opening
\renewcommand{\opening}[1]{\thispagestyle{firstpage}%
    \ifx\@empty\fromaddress
        %{\raggedleft\@date\par}%
    \else  % home address
        {\raggedleft
            \begin{tabular}{l@{}}\ignorespaces
            \fromaddress \\ *[1\parskip]%
            %\@date
            \end{tabular}\par
        }%
     \fi
     \vspace{-6\parskip}
     \@date \vspace{2\parskip}\\
     {\raggedright \toname \\ \toaddress \par}%
     \vspace{1\parskip}%
     \ifthenelse{\equal{\@subject}{}}{}{\@subject\par}
     \vspace{1\parskip}%
     #1\par\nobreak
}

% we push closing to the left
\renewcommand{\closing}[1]{\par\nobreak\vspace{\parskip}%
    \stopbreaks
    \noindent
    \parbox{0.4\textwidth}{\raggedright
    \ignorespaces #1\\[4\medskipamount]%
    \ifx\@empty\fromsig
        \fromname
    \else \fromsig 
    \fi\strut}%
    \par
}
